Expos\'ia: Teaching and Assessment of Academic Writing Skills for Research Project Proposals and Peer Feedback

We present Expos\'ia, the first public dataset that connects writing and feedback in higher education, enabling research on educationally grounded computational approaches to teaching and evaluating academic writing. Expos\'ia includes student research project proposals and peer and instructor feedback consisting of comments and free-text reviews. The dataset was collected in the "Introduction to Scientific Work" course of the Computer Science. Expos\'ia reflects the multi-stage nature of the academic writing process that includes drafting, receiving feedback, and revising the writing based on the feedback received. Both the project proposals and peer feedback are accompanied by human assessment scores based on a fine-grained, pedagogically-grounded schema for writing and feedback assessment that we develop. We use Expos\'ia to benchmark state-of-the-art large language models (LLMs) on two tasks: automated scoring of (1) the proposals and (2) the student reviews. We find that the two tasks are best served by different LLMs. Furthermore, closed-source models consistently outperform open-weight models, motivating further research on improving the performance of open-weight models preferred in classroom settings. Finally, we establish that a prompting strategy that scores multiple aspects of the writing together is the most effective, paving the way for more effective classroom deployment of modern LLMs.

==> table/rubric_small.tex <==
\ignore{
\begin{table*}[t]
\centering
{
\setlength{\tabcolsep}{1mm}

\begin{tabular}{@{}l l >{\raggedright\arraybackslash}p{0.70\textwidth} c@{}}
\toprule
\textbf{Code} & \textbf{Rubric} & \textbf{Description} & \textbf{\#Crit.} \\
\midrule

% --- Exposé header row ---
\multicolumn{4}{@{}l}{\textbf{Exposé}}\\[-2pt]
\addlinespace[1pt]

LA & Lang./Quality & Assessment of language quality and structural coherence of the text. & 2 \\
ME & Metadata & Evaluation of title appropriateness and creativity. & 2 \\
ST & Form/Structure & Evaluation of document formatting and structural requirements. & 2 \\
MO & Motivation & Assessment of problem identification, context establishment, and research question formulation. & 7 \\
AP & Approach & Assessment of state of the art analysis, theoretical framework. & 8 \\
MD & Methodology & Assessment of the methodology. & 7 \\
SC & Schedule & Assessment of project timeline structure, completeness, and realism. & 4 \\
BI & Bibliography & Assessment of bibliography consistency and literature relevance. & 2 \\
AD & Addt'l points & Add points for great submissions or deduct points for major mistakes. & 2 \\

\midrule

% --- Review header row ---
\multicolumn{4}{@{}l}{\textbf{Review}}\\[-2pt]
\addlinespace[1pt]

SC & Structure/Clarity & Assessment of overall structure and clarity. & 2 \\
LG & Language & Assessment of language quality and tone. & 2 \\
FU & Feed Up & Assessment of learning goals and success criteria. & 2 \\
FB & Feed Back & Assessment of feedback quality and knowledge transfer. & 6 \\
FF & Feed Forward & Assessment of future learning guidance. & 2 \\
CQ & Content Quality & Assessment of content accuracy and usefulness. & 3 \\
ER & Errors & Assessment of potential errors and issues in feedback. & 5 \\
AD & Addt'l points & Add points for great reviews or deduct points for major mistakes. & 2 \\

\bottomrule
\end{tabular}
}
\caption{Exposé and review grading rubrics. The last column shows the number of criteria in the rubric.}
\label{tab:expose_review_rubrics}
  \vspace{-4mm}

\end{table*}
}



